B-CONCORD -- A scalable Bayesian high-dimensional precision matrix estimation procedure

Sparse estimation of the precision matrix under high-dimensional scaling constitutes a canonical problem in statistics and machine learning. Numerous regression and likelihood based approaches, many frequentist and some Bayesian in nature have been developed. Bayesian methods provide direct uncertainty quantification of the model parameters through the posterior distribution and thus do not require a second round of computations for obtaining debiased estimates of the model parameters and their confidence intervals. However, they are computationally expensive for settings involving more than 500 variables. To that end, we develop B-CONCORD for the problem at hand, a Bayesian analogue of the CONvex CORrelation selection methoD (CONCORD) introduced by Khare et al. (2015). B-CONCORD leverages the CONCORD generalized likelihood function together with a spike-and-slab prior distribution to induce sparsity in the precision matrix parameters. We establish model selection and estimation consistency under high-dimensional scaling; further, we develop a procedure that refits only the non-zero parameters of the precision matrix, leading to significant improvements in the estimates in finite samples. Extensive numerical work illustrates the computational scalability of the proposed approach vis-a-vis competing Bayesian methods, as well as its accuracy.

==> main_body.tex <==
\section{Introduction}

\noindent
High dimensional multivariate datasets, where the number of variables $p$ is comparable or much larger than the 
number of samples $n$, are omnipresent in modern scientific applications. One of the fundamental quantities that 
can help understand the complex network of relationships in these multivariate datasets is the covariance matrix 
$\Sigma$ of the variables. In high-dimensional settings, the sample covariance matrix $S$ of the observations is 
typically not a good estimator. The central issue is that there is $O(p^2)$ unknown parameters in the covariance 
matrix. Hence, a sample size of $n << p$ is not enough to obtain a good estimator, unless reducing the effective 
number of parameters are made. A common and popular approach for parameter reduction is to induce sparsity in 
the covariance matrix, its inverse (the precision matrix), or an appropriate function such as its Cholesky factor. 

Note that the $(i,j)^{th}$ entry of the precision matrix $\mathbf{\Omega} = \mathbf{\Sigma}^{-1}$ are proportional to the partial 
correlation between the $i^{th}$ and $j^{th}$ variable. In many applications, it is often reasonable to assume that there are 
only a few significant partial correlations and the other partial correlations are negligible in comparison. Hence, it is natural 
to induce sparsity in the precision matrix $\mathbf{\Omega}$ for these applications. The sparsity structure in 
$\mathbf{\Omega}$ can be conveniently represented in terms of a {\it partial correlation graph} $G$, whose vertices are the 
$p$ variables, and edge $(i,j)$ exists only if the partial correlation between the $i^{th}$ and $j^{th}$ variables is non-zero. 
When the underlying distribution is multivariate Gaussian, $\Omega_{ij} = 0$ additionally implies that $i^{th}$ and $j^{th}$ 
variables are conditionally independent given the other variables. Hence, in the Gaussian setting, these partial 
correlation graphs encode conditional independencies, and the corresponding models are called {\it Gaussian 
graphical models}.  

Several frequentist approaches have been developed for sparse precision matrix estimation. See 
\cite{Meinshausen:Buhlmann:2006, yuan2007model, friedman2008sparse, peng2009partial, CLL:2011, khare2015convex} 
and the references therein to name just a few. These approaches obtain sparse estimates of $\mathbf{\Omega}$ by 
minimizing the sum of an appropriate loss function and a sparsity inducing penalty function (such as the $\ell_1$-norm of 
$\mathbf{\Omega}$) and can be broadly classified into three groups. Likelihood based approaches, such as the graphical lasso 
\cite{friedman2008sparse} use the negative Gaussian likelihood as the loss function. Regression based approaches such 
as \cite{Meinshausen:Buhlmann:2006, peng2009partial, khare2015convex} use the fact that the $i^{th}$ row of 
$\mathbf{\Omega}$ (suitably normalized) is the vector of (population) least squares coefficients for regressing the $i^{th}$ 
variables against all the other variables in the dataset. They use the aggregated regression error sum of squares for each 
variable as the loss functions. Finally, other approaches such as \cite{CLL:2011} use loss functions which are connected 
neither to the Gaussian likelihood nor the regression based interpretation of $\mathbf{\Omega}$. 

The main challenge in sparse precision matrix estimation is selection of the partial correlation graph (sparsity pattern in 
$\mathbf{\Omega}$). For this task, a positive definite estimator of the inverse covariance matrix is not necessarily required. In 
fact, all (frequentist) regression based methods (such as 
\cite{Meinshausen:Buhlmann:2006, peng2009partial, khare2015convex}) and some likelihood free methods such as 
\cite{CLL:2011} focus on estimating the sparsity pattern in $\mathbf{\Omega}$, and do notimpose the constraint of positive 
definiteness on the inverse covariance matrix in their respective algorithms for mainly computational scalability reasons, but 
perform well in terms of network selection both in finite sample and asymptotic settings . 

To summarize, for the purposes of selecting the partial correlation graph, the regression based approaches enjoy two 
significant advantages compared to the (Gaussian) likelihood based approaches.  First, they do not inherently need to impose 
the positive definite constraint on $\mathbf{\Omega}$. This fact, along with the quadratic nature of the objective function, can 
be leveraged to decrease the computational complexity per iteration by an order of magnitude. Second, the regression 
interpretation of entries of $\mathbf{\Omega}$ does not depend on Gaussianity. Hence, regression based methods are more 
robust to deviations from Gaussianity. See \cite{khare2015convex} for more details. 

The Bayesian paradigm offers the advantage of natural uncertainty quantification through the posterior. Several Bayesian 
counterparts to the penalized (Gaussian) likelihood based methods have been proposed 
\cite{DLR:2011, wang2012bayesian, Cheng:Lenkoski:2012, Wang:2015}, but the main challenge for these Bayesian 
approaches is their scalability in high-dimensional settings. The spike-and-slab prior based approach of \cite{Wang:2015} 
is significantly scalable compared to previous approaches and performs well when the number of variables $p$ is in the lower 
hundreds, but struggles computationally when $p = 500$ or $p = 1000$ (see Section \ref{simulations} for more details). 

Our goal in this paper is to develop a {\it scalable} Bayesian approach for sparse precision matrix estimation in 
high-dimensional settings with thousands of variables by leveraging the regression based interpretation of $\mathbf{\Omega}$. 
We achieve this by combining the regression based generalized likelihood from \cite{khare2015convex} with a spike-and-slab 
prior to obtain a generalized posterior distribution for the precision matrix $\mathbf{\Omega}$. We then derive the induced 
posterior distribution on the space of sparsity patterns. These posterior probabilities are available in closed form (up to a 
normalizing constant) and scan be used to assess uncertainty for sparsity selection. Under standard regularity assumptions, 
we establish high-dimensional sparsity selection for this pseudo-posterior distribution on sparsity patterns. To the best of our 
knowledge, similar consistency results are not available for the Gaussian likelihood based approaches mentioned above. 
Through detailed simulations, we demonstrate that our method is computationally {\it substantially faster} than the state-of-the-
art Gaussian likelihood based Bayesian approach in \cite{Wang:2015} by orders of magnitude, while maintaining or improving 
statistical accuracy.  

The rest of the paper is organized as follows. We provide some background material about the regression based generalized 
likelihood in in Section \ref{background}. Our generalized likelihood based Bayesian approach for sparsity selection in the 
precision matrix is developed in Sections \ref{generalized:likelihood:spike:slab} and \ref{posterior:computation:gibbs:sampler}. 
While sparsity selection is our main goal, we also address the subsequent goal of computationally efficient estimation of the 
magnitudes of the non-zero entries of $\mathbf{\Omega}$ and corresponding issues of bias correction in 
Section \ref{refitting:technique}. High-dimensional selection consistency and convergence rates are established in 
Section \ref{sec:consistency}. Sections \ref{simulations} rigorously evaluates the finite sample computational and 
statistical performance of the proposed approach on simulated datasets. The proofs of the technical results are provided in a 
Supplemental Document. 



\section{Background: Regression based generalized likelihood} \label{background}

\noindent
We begin by providing some background and motivation for the regression based generalized likelihood in 
\cite{khare2015convex}. Let $\mathcal{Y} :=\left(\{\mathbf{y}_{i:}\}_{i=1}^{n}\right)$ denote $i.i.d$ observations from a 
$p$-variate (continuous) distribution, with mean $\boldsymbol{0}$ and covariance matrix $\mathbf{\Omega}^{-1}$.  Let 
$\mathbf{S}$ denote the sample covariance matrix of the observations. In the frequentist setting, one of the standard 
methods to achieve a sparse estimate of $\bf{\Omega}$ is to minimize an objective function, comprised of the (negative) 
Gaussian log-likelihood and an $\ell_1$-penalty term for the off-diagonal entries of $\bf{\Omega}$, over the space of 
positive definite matrices. Equivalently, one can maximize the following weighted Gaussian likelihood: 
\begin{equation}\label{glasso}
\text{exp}\left( -\frac{n}{2} \left\{   \text{tr} \left( \mathbf{\Omega} \mathbf{S} \right) - \text{log det}\ \mathbf{\Omega} + 
\frac{\lambda}{n} \mathop{\sum\sum}\limits_{1\le j \le k \le p} {\left| \omega_{jk}  \right|}  \right\}\right). 
\end{equation}

\noindent
This approach and its variants are known as the {\it graphical lasso}, see 
\cite{yuan2007model, friedman2008sparse, banerjee2008model}. The function in (\ref{glasso}) can also be 
regarded as the posterior density of $\mathbf{\Omega}$ (up to proportionality) under Laplace priors for the off-diagonal entries, leading 
to a Bayesian inference and analysis in \cite{wang2012bayesian}. Due to the constraint of positive definite definiteness on 
$\mathbf{\Omega}$, and the structure of the Gaussian likelihood, each iteration of the optimization algorithms for graphical lasso or the 
MCMC algorithms for it's Bayesian counterparts involves inversion of $(p-1)\times (p-1)$ matrices in each iteration, which can 
be computationally very intensive when $p$ is large~\footnote{Many useful methods to improve the computational 
performance of graphical lasso have been proposed, such as \cite{mazumder2012graphical} and \cite{HSDR:2014}. However, these 
methods provide substantial improvements only under certain assumptions on the number and size of the connected 
components of the graph implied by the zeros in the minimizer, and/or still involve inversions of $(p-1) \times (p-1)$ matrices.}.

To address this problem in the frequentist setting, several works (see \cite{peng2009partial}, \cite{khare2015convex}) have 
considered replacing the Gaussian likelihood by a regression based generalized likelihood. Note that $-\frac{\omega_{jk}}
{\omega_{jj}}$ is the regression coefficient of $\mathbf{y}_{k:}$ when we regress $\mathbf{y}_{j:}$ on all other variables, and 
$\frac{1}{\omega_{jj}}$ is the residual variance. This is true even in non-Gaussian settings. \cite{peng2009partial} use this 
interpretation to define a generalized likelihood in terms of the (negative) exponent of the combined weighted squared error 
loss associated with all these regressions (corresponding to all $p$ variables) as follows. 
\begin{equation} \label{eq1}
\text{exp} \left( -\sum\limits_{j=1}^{p} {\omega_{jj}} \left\{ \sum\limits_{i=1}^{n} {\left( y_{ij} - \sum\limits_{k\ne j}
-{\frac{\omega_{jk}}{\omega_{jj}}y_{ik}} \right)^2} \right\} - \sum\limits_{j=1}^p \frac{n}{2} {\text{log}\omega_{jj}} \right).
\end{equation}

\noindent
Under Gaussianity, the expression in (\ref{eq1}) corresponds to the product of the conditional densities of each variable given 
all the other variables in the dataset, and corresponds to Besag \cite{Besag:1975}'s pseudo-likelihood. \cite{peng2009partial} 
develop the SPACE algorithm which obtains a sparse estimator for $\mathbf{\Omega}$ by minimizing an objectiv function 
consisting of the (negative) log generalized likelihood and an $\ell_{1}$ penalty term for off-diagonal entries of 
$\mathbf{\Omega}$. However, this objective function is not jointly convex, which can lead to serious convergence issues for 
the corresponding minimization algorithm. 

\cite{khare2015convex} address this issue by appropriately reweighting each of the $p$ regression terms in the exponent of 
(\ref{eq1}) and combining it with an $\ell_1$ penalty term to obtain a regression based loss function which is jointly convex in 
$\mathbf{\Omega}$. This loss function, refered by \cite{khare2015convex} as the CONCORD objective function, is given by
\begin{equation} \label{concord likelihood}
\begin{split}
Q_{con}\left(\mathbf{\Omega} \right) &= -n\sum\limits_{j=1}^{p}{\text{log}\omega_{jj}} + \frac{1}{2}\sum\limits_{j=1}^{p}
{\sum\limits_{i=1}^{n}{\left( \omega_{jj}y_{ij} + \sum\limits_{k \ne j}{\omega_{jk}y_{ik}} \right)^2}} + \lambda \mathop{\sum\sum}
\limits_{1 \le j < k \le p}|\omega_{jk}|  \\
&= -n\sum\limits_{j=1}^{p}{\text{log}\omega_{jj}} + \frac{n}{2} \text{tr} \left( \mathbf{\Omega}^2\mathbf{S}\right) + \lambda 
\mathop{\sum\sum}\limits_{1 \le j < k \le p}|\omega_{jk}|. 
\end{split}
\end{equation}

\noindent
Here $\mathbf{S}$ denotes the sample covariance matrix. The joint convexity of $Q_{con}$ can be used to show that the 
coordinatewise minimization algorithm always converges to a global minimum. Note that both \cite{peng2009partial} and 
\cite{khare2015convex} relax the parameter space of $\mathbf{\Omega}$ from positive definite matrices to symmetric matrices with 
positive diagonal entries. The primary purpose of this relaxation is computational. Combined with the quadratic nature of the 
objective function, this relaxation leads to an {\it order of magnitude decrease in computational complexity} as compared to 
graphical lasso based approaches. Note that given the $\text{log det} \mathbf{\Omega}$ term in the Gaussian likelihood, such a 
parameter relaxation will not work for the graphical lasso. 

While the resulting minimizer may not be positive definite, its sparsity structure can be used to address the 
primary goal/challenge of selecting the sparsity pattern in $\mathbf{\Omega}$. \cite{khare2015convex} establish 
high-dimensional sparsity selection consistency of this approach, and also demonstrate that the CONCORD approach can 
outperform graphical lasso when the underlying data is not generated from a multivariate Gaussian distribution. This 
robustness is somewhat expected, since the regression based interpretation of $\mathbf{\Omega}$ does not depend on Gaussianity. 



\section{Proposed framework: Bayesian CONCORD for sparsity selection}

\noindent
The goal of this section is to develop a Bayesian framework for sparse precision matrix estimation which couples the 
computational advantage and robustness offered by the regression based approach with the natural uncertainty 
quantification offered by the Bayesian paradigm. 

Many modern frequentist methods obtain estimates by minimizing an objective function which is the sum of the negative 
log-likelihood and an appropriate penalty function. As exemplified in Section \ref{background}, many methods, however, 
replace the log-likelihood by a data-based loss function for computational and/or robustness purposes. In the Bayesian 
paradigm, a similar approach can be used, where the likelihood is replaced by an appropriate data-based positive weight 
function or generalized likelihood. While the generalized likelihood is not necessarily a probability density, as long as the 
product of the generalized likelihood and the prior density is integrable over the parameter space, one can construct a 
pseudo-posterior distribution and do Bayesian inference and uncertainty quantification. See 
\cite{ventura2016pseudo, PNNC:2017, Miller:2019} and the references therein. Of course, it is crucial to rigorously 
evaluate the properties of any such generalized likelihood based approach both in asymptotic settings and through 
finite sample simulations.  

In the context of network estimation, \cite{PNNC:2017} use \cite{Besag:1975}'s pseudo-likelihood to develop a 
Bayesian Markov network estimation procedure for {\it jointly discrete} random variables. Our focus in this paper is partial 
correlation graph estimation for {\it jointly continuous} random variables. We will develop a regression based generalized 
likelihood for this purpose based on the CONCORD objective function in (\ref{concord likelihood}). In the special Gaussian 
setting, generalized likelihood (see (\ref{eq2}) below) is related to, but different from the pseudo-likelihood of 
\cite{Besag:1975}. 

Note that the first two terms (non-penalty part) of the CONCORD objective function $Q_{con}$ in (\ref{concord likelihood}) 
consist of a weighted error sum of squares for regressing each variable against all the others, and an additional logarithmic 
term for the conditional variance terms. Together, these two terms provide a regression based loss function which measures 
how closely the parameter value reflects the observed data. We define the CONCORD generalized likelihood as the 
(negative) exponential of the sum of these two terms as follows. 
\begin{equation} \label{eq2}
\mathcal{L}_{CONCORD} ({\bf \Omega}) := \exp \left( - \frac{1}{2}\sum\limits_{j=1}^{p}
{\sum\limits_{i=1}^{n}{\left( \omega_{jj}y_{ij} + \sum\limits_{k \ne j}{\omega_{jk}y_{ik}} \right)^2}} + n \sum\limits_{j=1}^p 
\log \omega_{jj} \right). 
\end{equation}

\noindent
As in the frequentist regression based setting, for computational reasons, we will relax the parameter space for $\mathbf{\Omega}$ 
from the space of positive definite matrices to $\mathbf{\mathbb{M}}_{p}^{+}$, the space of all $p \times p$ matrices with 
positive diagonal entries. Recall that our principal goal is sparsity selection, and as we show below, a generalized 
posterior distribution over the space of all possible sparsity patterns can be obtained as used for Bayesian inference. 
Furthermore, we will rigorously evaluate the asymptotic and finite sample statistical properties of this generalized posterior in 
subsequent sections, and demonstrate its effectiveness. We will also show that on the computational side, as in the 
frequentist setting, the relaxation of the parameter space, along with the straightforward quadratic and logarithmic 
expressions in the CONCORD generalized likelihood, lead to a substantial improvement in performance 
as compared to the state-of-the-art Gaussian likelihood based method in \cite{Wang:2015}. With the generalized 
likelihood in hand, we now focus on choosing the prior distribution. 

 
\subsection{Spike and Slab Prior} \label{generalized:likelihood:spike:slab}

\noindent
For a sparsity based Bayesian analysis, one standard choice of prior is the spike and slab prior (first pioneered by 
\cite{mitchell1988bayesian}), which is a mixture of a point mass at zero and an appropriate continuous probability distribution 
every where else. We choose such a prior for every off-diagonal entry of ${\bf \Omega} \in \mathbf{\mathbb{M}}_p^+$. In 
particular 
\begin{equation}\label{spikeslab}
\omega_{jk} \sim (1-q)I_{\{0\}}(\omega_{jk}) + q \phi_{\lambda_{jk}} (\omega_{jk}) I_{\mathbb{R} \setminus \{0\}}(\omega_{jk}) 
\end{equation}

\noindent
independently for every $1 \leq j < k \leq p$, where $\phi_\lambda$ denotes the normal density with mean zero and 
variance $1/\lambda$. Recall that as in the frequentist generalized likelihood based approaches for sparsity selection, we 
are relaxing the positive definite constraint on ${\bf \Omega}$ We put an independent Exponential$(\gamma)$ prior on all the 
diagonal entries of ${\bf \Omega}$. Hence the (shrinkage) hyperparameters are $\{\lambda_{jk}\}_{1 \leq j < k \leq p}$ and 
$\gamma$. We will discuss the choice of these hyperparameters in Remark \ref{hyperparameter:selection}. 

We now introduce additional notation for ease of exposition, in particular for the asymptotic analysis in 
Section \ref{sec:consistency}. Let 
\begin{equation} \label{theta}
{\boldsymbol \xi} = (\omega_{21}, \omega_{31}, \omega_{32}, \cdots, \omega_{p,p-2}, \omega_{p,p-1}) 
\end{equation}

\noindent
denote the collection of off-diagonal entries of the symmetric matrix ${\bf \Omega}$. Let $\boldsymbol{l} \in 
\{0,1\}^{{p \choose 2}}$ be a generic sparsity pattern for ${\boldsymbol \xi}$. There are $2^{{p \choose 2}}$ such 
sparsity patterns. For example, when $p = 3$, there are ${3 \choose 2} = 3$ off-diagonal entries, and the 
$2^{{p \choose 2}} = 8$ possible sparsity patterns in the off-diagonal entries are given by 
\begin{align*}
& (0,0,0), \; (1,0,0), \; (0,1,0), \; (0,0,1)\\
& (1,1,0), \; (1,0,1), \; (0,1,1), \; (1,1,1). 
\end{align*}

\noindent
For every sparsity pattern $\boldsymbol{l}$, let $d_{\boldsymbol{l}}$ be the density (number of non-zero entries) of 
$\boldsymbol{l}$, and $\mathcal{M}_{\boldsymbol{l}}$ be the space where ${\boldsymbol \xi}$ varies when 
restricted to follow the sparsity pattern $\boldsymbol{l}$. in the $p=3$ example discussed above, $d_{(0,0,0)} = 0$ and 
$d_{(1,0,0)} = 1$. 

Using straightforward calculations, the independent spike-and-slab priors for the off-diagonal entries (specified in 
(\ref{spikeslab}), can be alternatively represented as a hierarchical prior distribution as follows. 
\begin{equation} \label{hierarchical prior 1}
\pi \left( {\boldsymbol \xi} | \boldsymbol{l}\right) = \frac{|\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}}|^{\frac{1}{2}}}{\left(2\pi \right)^{\frac{d_{\boldsymbol{l}}}{2}}} \exp \left(-\frac{{\boldsymbol \xi}'\mathbf{\Lambda}{\boldsymbol \xi}}{2} \right)I_{\left( {\boldsymbol \xi} \in \mathcal{M}_{\ell}\right)},
\end{equation}

\noindent
where $\mathbf{\Lambda}$ is a diagonal matrix with diagonal entries $(\lambda_{jk})_{1 \leq j < k \leq p}$, and 
$\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}}$ is a sub-matrix of $\mathbf{\Lambda}$ obtained after removing the 
rows and columns corresponding to the zeros in ${\boldsymbol \xi} \in \mathcal{M}_{\boldsymbol{l}}$. In other words, 
given the sparsity pattern ${\boldsymbol{l}}$, the non-zero entries of ${\boldsymbol \xi}$ follow a 
$d_{\boldsymbol{l}}$-dimensional multivariate normal distribution with mean ${\bf 0}$ and covariance matrix 
$\Lambda_{\boldsymbol{l}\boldsymbol{l}}^{-1}$. The marginal distribution of $\boldsymbol{l}$ is given by 

\begin{equation}\label{hierarchical prior 2}
\pi(\boldsymbol{l}) \propto \begin{cases} 
q^{d_{\boldsymbol{l}}}(1-q)^{\binom{p}{2} - d_{\boldsymbol{l}}} & d_{\boldsymbol{l}} \leq \tau,\\
0 & d_{\boldsymbol{l}} > \tau. 
\end{cases}
\end{equation}
which puts zeros mass on {\it unrealistic sparsity patterns}, i.e., sparsity patterns with more than $\tau$ non-zero entries. Later, in our theoretical analysis, we will discuss appropriate values for $\tau$. 

\noindent
Using (\ref{hierarchical prior 1}) and (\ref{hierarchical prior 2}), the marginal prior distribution on ${\boldsymbol \xi}$ can be 
obtained as a mixture of multivariate normal distributions as follows. 
\begin{equation}\label{prior on theta}
\begin{split}
\pi\left( {\boldsymbol \xi} \right)  = \sum\limits_{ \boldsymbol{l} \in \mathcal{L}}\pi\left({\boldsymbol \xi} | \boldsymbol{l}\right)\pi\left(\boldsymbol{l}\right)
&\propto \sum\limits_{ \boldsymbol{l} \in \mathcal{L}} q^{d_{\boldsymbol{l}}}(1-q)^{\binom{p}{2} - d_{\boldsymbol{l}}} \left\{ \frac{|\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}}|^{\frac{1}{2}}}{\left(2\pi \right)^{\frac{d_{\boldsymbol{l}}}{2}}} \exp \left(-\frac{{\boldsymbol \xi}'\mathbf{\Lambda}{\boldsymbol \xi}}{2} \right)I_{\left( {\boldsymbol \xi} \in \mathcal{M}_{\ell}\right)} \right\}. 
\end{split}
\end{equation}

\noindent
Note that the vector ${\boldsymbol \xi}$ only incorporates the off-diagonal entries of $\mathbf{\Omega}$. Regarding the 
diagonal entries, we define $\boldsymbol{\delta}$ to be the vector of all diagonal elements $\mathbf{\Omega}$, i.e.
\begin{equation}\label{delta}
\boldsymbol{\delta} = \left( \omega_{11}, ..., \omega_{pp}\right). 
\end{equation}

\noindent
Note that we are assigning an independent Exponential($\gamma$) prior on each coordinate of $\boldsymbol{\delta}$, i.e,
\begin{equation}\label{prior on delta}
\pi\left( \boldsymbol{\delta} \right) \propto \exp \left( -\gamma \boldsymbol{1}'\boldsymbol{\delta} \right) I_{\mathbb{R}_{+}^{p}}
\left( \boldsymbol{\delta} \right).
\end{equation}

\noindent
We will come back to the $({\boldsymbol \xi}, \boldsymbol{\delta})$ notation above in the high-dimensional consistency analysis 
in Section \ref{sec:consistency}. 

\subsection{Posterior Computation} \label{posterior:computation:gibbs:sampler}

\noindent
Combining (\ref{eq2}) and (\ref{spikeslab}), it is easy to check that the generalized posterior density of ${\bf \Omega}$ is given 
by 
\begin{eqnarray}
\pi \left\{ \left( \mathbf{\Omega} \right)| \mathcal{Y}\right\} \propto & \ \text{exp} \left( n\sum\limits_{j=1}^{p}{\text{log}\omega_{jj}} - \frac{n}{2}\text{tr}\left( \mathbf{\Omega}^2\mathbf{S}\right) - 
\lambda \mathop{\sum\sum}\limits_{1 \le j < k \le p}\frac{\omega_{jk}^2}{2} - \lambda \sum_{j=1}^p\omega_{jj}\right) 
\nonumber\\
\times & \prod \limits_{1 \le j < k \le p} \left( I_{\{0\}} (\omega_{jk}) + \frac{q\sqrt{\lambda_{jk}}}{(1-q)\sqrt{2 \pi}} 
I_{\mathbb{R} \setminus \{0\}}(\omega_{jk}) \right). \label{BSSC posterior}
\end{eqnarray}

\noindent
The generalized posterior density in (\ref{BSSC posterior}) is intractable in the sense that it is not feasible to draw exact 
samples from such density. However, we will use the conditional posterior density of each element $\omega_{jk}$ of 
$\mathbf{\Omega}$, $1 \leq j \leq k \leq p$, given the remaining elements denoted by $\mathbf{\Omega}_{-(jk)}$, to introduce 
an entry wise Gibbs sampler that can generate approximate samples from the generalized posterior density in 
(\ref{BSSC posterior}). In order to compute the conditional posterior density of the off-diagonal elements $\omega_{jk}$, for 
$1 \le j \leq k \le p$, we first note that 
\begin{equation}\label{eq6}
 n\text{tr}\left( \mathbf{\Omega}^2\mathbf{S}\right)
=\sum\limits_{i=1}^{n}\| \left( \mathbf{\Omega} \mathbf{y}_{i:}\right) \|^2
= \sum\limits_{i=1}^{n}{\sum\limits_{j=1}^{p}{\left( \sum\limits_{k=1}^{p}{\omega_{jk}y_{ik}}\right)^2}} =\sum\limits_{j=1}^{p} \| 
\left( \sum\limits_{k=1}^{p}{\omega_{jk} \mathbf{y}_{:k}}\right) \|^2, 
\end{equation}

\noindent
Thus, in view of (\ref{eq6}), straightforward algebra shows that
\begin{equation*}
\begin{split}
\pi (\omega_{jk}| \mathbf{\Omega}_{-(jk)}, \mathcal{Y}) &\propto \exp \left\{ -\frac{n}{2} \left( a_{jk}\omega_{jk}^{2} + 2 b_{jk}
\omega_{jk}\right)\right\} \left( I_{\{0\}} (\omega_{jk}) + \frac{q\sqrt{\lambda}}{(1-q)\sqrt{2 \pi}} 
I_{\mathbb{R} \setminus \{0\}}(\omega_{jk}) \right)\\
&=I_{\{0\} }(\omega_{jk}) + c_{jk}\frac{\sqrt{na_{jk}}}{\sqrt{2\pi}} \exp\left\{ -\frac{na_{jk}}{2} \left( \omega_{jk} + 
\frac{b_{jk}}{a_{jk}}\right)^2\right\}I_{\mathbb{R} \setminus \{0\}}(\omega_{jk})
\end{split}
\end{equation*}

\noindent
with,
\begin{equation*}
\begin{split}
a_{jk} &= s_{jj} + s_{kk} + \frac{\lambda_{jk}}{n}, \quad \quad \quad 
b_{jk} = \sum_{k' \neq k} \omega_{jk'} s_{kk'} + \sum_{j' \neq j} \omega_{j'k} s_{jj'}\\
c_{jk} &= \frac{q \sqrt{\lambda_{jk}}}{(1-q) \sqrt{na_{jk}}}\exp\left( \frac{nb_{jk}^2}{2a_{jk}}\right).
\end{split}
\end{equation*}
now, by letting $p_{jk} = \frac{c_{jk}}{1+c_{jk}}$, we can write
\begin{equation}\label{cond. omegas_jk BSSC}
\begin{split}
(\omega_{jk}| \mathbf{\Omega}_{-(jk)}, \mathcal{Y}) \sim (1-p_{jk})I_{\{0\}}(\omega_{jk}) + p_{jk}N(-\frac{b_{jk}}{a_{jk}}, \frac{1}{na_{jk}})I_{\mathbb{R} \setminus \{0\} }(\omega_{jk}), \quad \quad 1 \le j < k \le p.
\end{split}
\end{equation}

Moreover, the diagonal elements $\omega_{jj}$, are conditionally independent and the conditional density of $ \omega_{jj}$ given $\mathbf{\Omega_{-(jj)}}$, for $1 \le j \le p$, is given by
\begin{equation}\label{cond. diags BSSC}
\begin{split}
f(\omega_{jj}| \mathbf{\Omega}_{-(jj)}, \mathcal{Y}) \propto \omega_{jj}^{n}\text{exp}\left\{ -\omega_{jj}^{2}\left( \frac{n}{2} s_{jj}
\right) - \omega_{jj}\left( \lambda_{jk} + n b_j \right) \right\},
\end{split}
\end{equation}

\noindent
where 
$$
b_j = \sum_{j' \neq j} \omega_{jj'}' s_{jj'}. 
$$

\noindent
Note that the density in \ref{cond. diags BSSC} is not a standard density, but using the fact that it has a unique mode at
\begin{equation}\label{mode of diag dist}
\frac{-(\lambda_{jk} + nb_j) + \sqrt{(\lambda + nb_j)^2 + 4n^2 s_{ii}^k}}{2n s_{ii}^k}, 
\end{equation}

\noindent
one can use a discretization technique to generate samples from it. However, we have observed in our simulations that the 
density in (\ref{cond. diags BSSC}) puts most of its mass around the mode. As a result, when appropriate, one can simply 
approximate it using a degenerate density with a point mass at it's mode, given in \ref{mode of diag dist}. This approximation 
allows faster implementation of our algorithm without much sacrificing on it's accuracy. Using the distributions in 
(\ref{cond. omegas_jk BSSC}) and (\ref{cond. diags BSSC}), we build a component-wise Gibbs sampler to generate 
approximate samples from the joint posterior density in (\ref{BSSC posterior}). Given the current value of $\mathbf{\Omega}$, one iteration of this Gibbs sampler, which henceforth is referred to as Bayesian Spike and Slab Concord (BSSC), is described in Algorithm \ref{GibbsBSSC}.
\begin{algorithm}
\caption{Entry wise Gibbs Sampler for BSSC}
\begin{algorithmic}
\Procedure{BSSC}{$\mathbf{S}$}\Comment{Input the data}
\For{$j=1, ..., p-1$}
\For{$k=j+1, ..., p$}
\State $\omega_{jk} \sim (1-p_{jk})I_{\{0\} }(\omega_{jk}) + p_{jk}N(-\frac{b_{jk}}{a_{jk}}, \frac{1}{a_{jk}})I_{\mathbb{R} \setminus 
\{0\}}(\omega_{jk})$
\EndFor
\EndFor
\For{$j=1, ..., p$}
\State $\omega_{jj} \gets \frac{-(\lambda_{jk} + n\mathbf{\Omega}_{-jj}'\mathbf{S}_{-jj}) + \sqrt{(\lambda_{jk} + 
nb_j)^2 + 4n^2 s_{ii}^k}}{2n s_{ii}^k}$
\EndFor
\State \textbf{return} $ \mathbf{\Omega}$\Comment{Return $\mathbf{\Omega}$}
\EndProcedure
\end{algorithmic}\label{GibbsBSSC}
\end{algorithm}

Let $\left\{ \hat{\mathbf{\Omega}}^{(t)} \right\}_{t=1}^T$ denote the iterates obtained by running the Gibbs sampler (with sufficient 
burn-in). For each $1 \leq j < k \leq p$, we compute the proportion of times the corresponding entry was chosen to be 
non-zero, 
i.e.,
$$
\hat{p}_{jk} = \frac{1}{T} \sum_{t=1}^T 1_{\{\hat{\omega}_{jk}^{(t)} \neq 0\}}. 
$$

\noindent
If $\hat{p}_{jk}$ is greater than a pre-specified threshold $\upsilon \in (0,1)$, $(j,k)$, the $(j,k)^{th}$ entry is treated as non-zero 
in our estimated sparsity pattern for the precision matrix. Note that by the ergodic theorem $\hat{p}_{jk}$ converges to the 
posterior probability of $\omega_{jk}$ being non-zero as $T \rightarrow 0$. Hence, we are essentially classifying an entry as 
non-zero if the posterior probability of being non-zero is above $\upsilon$. We denote the resulting sparsity pattern estimate by 
$\hat{\boldsymbol{l}}_{\upsilon, BSSC}$, and use the threshold $\upsilon = 0.5$ in our experiments to obtain 
the {\it median probability model/sparsity pattern}. The user has the flexibility to use more conservative or relaxed threshold 
values based on his/her choice. 
\begin{Remark} (Selection of hyperparameters) \label{hyperparameter:selection}
Choice of the shrinkage hyperparameters $\{\lambda_{jk}\}_{1 \leq j < k \leq p}$ and $\{\gamma_j\}_{j=1}^p$, along with the 
mixing probability $q$ is an important task. Following 
\cite{park2008bayesian,wang2012bayesian}, we assign independent gamma priors 
on each shrinkage parameter $\lambda_{jk}$ and $\gamma_j$, i.e., 
\begin{align*}
& \lambda_{jk} \sim \text{Gamma}(r, s) \quad \quad \mbox{for} \quad 1 \leq j < k \leq p, 
& \gamma_j \sim \text{Gamma}(r, s) \quad \quad \mbox{for} \quad 1 \leq j \leq p 
\end{align*} 

\noindent
for some fixed $r, s > 0$. Straightforward calculations demonstrate that $\{\lambda_{jk}\}_{1 \leq j < k \leq p}, 
\{\gamma_j\}_{j=1}^p$ are conditionally mutually independent given $\mathbf{\Omega}, \mathcal{Y}$, i.e., 
\begin{align*}
& \lambda_{jk} \mid \mathbf{\Omega}, \mathcal{Y} \sim \text{Gamma}(r + 0.5, 0.5 \omega_{jk}^2+ s), 
& \gamma \mid \mathbf{\Omega}, \mathcal{Y} \sim \text{Gamma}(r + 1, \omega_{jj} + s). 
\end{align*}

\noindent
Since $\mathbb{E}\{\lambda_{jk} \mid \mathbf{\Omega}, \mathcal{Y}\} = \frac{r + 0.5}{0.5 \omega_{jk}^2+ s}$ and 
$\mathbb{E}\{\gamma_j \mid \mathbf{\Omega}, \mathcal{Y}\} = \frac{r + 1}{\omega_{jj} + s}$, this approach 
selects the respective shrinkage parameters based on the current $\omega$-values in a way that 
larger (smaller) entries are regularized less (more) on average. For the parameter $r$ and $s$ for the 
Gamma prior, in absence of any prior information, we recommend the non-informative choice $r=10^{-4}$ and 
$s=10^{-8}$, which is very close to a flat prior for the $\lambda$ and $\gamma$ values, and is based 
on the suggestions made in \cite{wang2012bayesian} of hyperparameter selection. In general, we have found 
that this choice works well in the experiments in Section \ref{simulations}. 

For the mixing probability $q$, our default choice is the objective choice $q = 1/2$. Based on the consistency results in 
Section \ref{sec:consistency}, one can use the choice $q = 1/p$ in really high-dimensional situations to further 
encourage sparser models. 
\end{Remark}

\subsection{Estimating magnitudes of non-zero entries: Correcting for bias using refitting} \label{refitting:technique}

\noindent
As mentioned previously, our main goal is sparsity selection in the precision matrix $\mathbf{\Omega}$. Sometimes, an 
estimate of the magnitude of the chosen non-zero entries of $\mathbf{\Omega}$ is also needed for downstream applications. 
Note that these estimates can be obtained from Algorithm \ref{GibbsBSSC}, and we establish the asymptotic accuracy/convergence rates of these estimates in high-dimensional settings in Theorem \ref{theorem (Estimation Consistency and Convergence Rate)}. However, in finite sample settings, these estimates 
are expected to be biased (estimates based on sparsity inducing regularization typically tend to be biased, see for example 
the literature on the debiased lasso in \cite{Zhang:Zhang:2014, Javanmard:Montanari:2014, VanDeGeer:2019}), and this is 
indeed supported by our simulations in Section \ref{simulations}. One way of addressing this problem in the penalized 
frequentist setting is to use an appropriate refitting step using the selected sparsity pattern (see for example 
\cite{ma2016joint}). In this section, we propose a Bayesian refitting step for obtaining debaised/improved estimates of the 
magnitudes of the non-zero entries of $\mathbf{\Omega}$ (as specified by the sparsity pattern obtained from Algorithm \ref{GibbsBSSC}). Figure \ref{fig:bias motivation} is an illustration of the effectiveness of the refitting technique which will be later introduced in this section. In the plot, we depict the estimation accuracy for one coefficient of a precision matrix of dimension $p=50$ and with sample sizes $n=100$ (subplot \ref{fig:bias motivation sub1}) and $n=1000$ (subplot \ref{fig:bias motivation sub2}). The posterior density of the coefficient was estimated using both BSSC and the refitting approach which are colored in red and blue, respectively. The true coefficient value is shown using the green vertical line. Figure \ref{fig:bias motivation} shows that the true coefficient is located withing the range of the estimated posterior density generated by the refitting approach. In Theorem \ref{estimation:consistency:refitted:posterior} we will theoretically establish the posterior estimation consistency of the refitting approach. In addition, later in section \ref{accuracy}, we will further demonstrate the numerical significance of the refitting approach in reducing the estimation error. 

\begin{figure}[h]
\centering
\caption{A scenario illustrating the problem of bias in estimating graphical models for one coefficient of a precision matrix with $p=50$, at two sample sizes $n=100$ in sub-plot (a), and $n=1000$ in sub-plot (b)}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=2in,width=3in,angle=0]{bias_motive_n_100}
  \caption{}
  \label{fig:bias motivation sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=2in,width=3in,angle=0]{bias_motive_n_1000}
  \caption{}
  \label{fig:bias motivation sub2}
\end{subfigure}
\label{fig:bias motivation}
\end{figure}


 Recall from the discussion at the end of Section \ref{posterior:computation:gibbs:sampler} that 
using the output of Algorithm \ref{GibbsBSSC}, for each $j \neq k$, we can compute the proportion of times the $(j,k)^{th}$ 
entry was chosen to be non-zero in the iterates (denoted by $\hat{p}_{jk}$). Let $\upsilon$ be the user specified threshold, and 
let 
$$
\hat{E} = \{ (j,k): \; \hat{p}_{jk} > \upsilon\}
$$

\noindent
denote the collection of indices classified as non-zero. Let $\hat{G}$ denote the graph with vertices $\{1,2, \cdots, p\}$ and 
edge set $\hat{E}$. In other words, $\hat{G}$ encodes the sparsity pattern of $\hat{\mathbf{\Omega}}$. Let 
$\mathbb{M}_{\hat{G}}$ defined by 
$$
\mathbb{M}_{\hat{G}} = \left\{ \mathbf{\Omega} \in \mathbb{M}_p^+: M_{ij} = 0 \mbox{ if } i \neq j, (i,j) \notin \hat{E} \right\}
$$

\noindent
denote the space of symmetric $p \times p$ matrices with positive diagonal entries which obey the sparsity pattern 
encoded in $\hat{G}$. Our goal now is to construct a debiased/improved estimate (and credible region) for 
$\mathbf{\Omega}$ lying in $\mathbb{M}_{\hat{G}}$ by specifying an appropriate prior distribution on $\mathbb{M}_{\hat{G}}$. 

An immediate question that might arise in the mind of the reader is that while the positive definite constraint can be relaxed for 
the purpose of estimating the sparsity pattern in $\mathbf{\Omega}$, this constraint should be imposed for estimating the 
magnitudes of the entries of $\mathbf{\Omega}$. One can certainly do this by further restricting to the space 
$\mathbb{P}_{\hat{G}}$ (which is defined to be the intersection of $\mathbb{M}_{\hat{G}}$ with positive definite matrices), 
specifying a prior on $\mathbb{P}_{\hat{G}}$, and then using the subsequent posterior distribution. This however leads to 
significant computational challenges and involves inversion of $p-1$ dimensional matrices. Hence, for computational reasons, 
we first construct our prior on $\mathbb{M}_{\hat{G}}$, and project the resulting estimator (and associated credible region) on 
the space of positive definite matrices by modifying the diagonal entries (see the end of this section for details). 

We start by specifying an improper prior distribution on $\mathbb{M}_{\hat{G}}$, and explain why we expect the resulting 
posterior distribution to lead to good estimators. We specify independent (improper) uniform priors on the the off-diagonal 
entries $\{\omega_{jk}\}_{(j,k) \in E}$ and for the diagonal entries we independently specify the following improper priors: 
\begin{equation}
\begin{split}
\pi(\omega_{jj}) &\propto \exp\left( n\omega_{jj} - n\log\omega_{jj}\right), \quad \omega_{jj} > 0, \quad \text{for} \quad 1 \leq j 
\leq p.
\end{split}
\end{equation}

\noindent
Then, the joint posterior distribution on $\mathbb{M}_{\hat{G}}$ is given by 
\begin{equation} \label{refitted:posterior:density}
\pi_{refitted} \left(\mathbf{\Omega}|\mathcal{Y} \right) \propto \exp\{n \text{tr}\left(\mathbf{\Omega}\right)-\frac{n}{2} \text{tr}
\left( \mathbf{\Omega}^2 \mathbf{S})\right\} \mbox{ for } \mathbf{\Omega} \in \mathbb{M}_{\hat{G}}. 
\end{equation}

\noindent
We refer to this posterior as the {\bf refitted posterior}, since this posterior is defined conditional on the sparsity pattern 
estimated from Algorithm \ref{GibbsBSSC} and encoded in $\hat{G}$. The following lemma addresses the propriety and 
unimodality of the posterior, and is proved in the Supplemental Document. 
\newtheorem{lem}{Lemma}
\begin{lem} \label{propriety}
If the degree of $\hat{G}$ (maximum number of edges shared by any vertex) is less than $n$, then the following holds. 
\begin{enumerate}
\item The refitted posterior density in (\ref{refitted:posterior:density}) can be normalized to a proper probability density. 
\item This refitted posterior density is log-concave, and has a unique mode. 
\end{enumerate}
\end{lem}

\noindent
The next lemma helps us understand why we expect the mode of the refitted posterior to be a good/improved estimator of 
$\mathbf{\Omega}$. 
\begin{lem} \label{optimizer}
Suppose $\mathbf{K} \in \mathbb{M}_{\hat{G}}$ and is invertible. Then 
$$
\mathbf{K} = \mbox{arg min}_{\mathbf{\Omega} \in \mathbb{M}_{\hat{G}}} \left\{ \frac{n}{2} \text{tr} \left( \mathbf{\Omega}^2 
\mathbf{K}^{-1} \right) - n \text{tr} (\mathbf{\Omega}) \right\}. 
$$
\end{lem}

\noindent
Suppose the true precision matrix $\mathbf{\Omega}_0 = \mathbf{\Sigma}_0^{-1}$ belongs to $\mathbb{M}_G$ for some graph 
$G$. Then, it follows from Lemma \ref{optimizer} that 
$$
\mathbf{\Omega}_0 = \mbox{arg min}_{\mathbf{\Omega} \in \mathbb{M}_G} \left\{ \frac{n}{2} \text{tr} \left( \mathbf{\Omega}^2 
\mathbf{\Sigma}_0 \right) - n \text{tr} (\mathbf{\Omega}) \right\}. 
$$

Note that under mild regularity assumptions the maximum entrywise difference between the sample covariance matrix and 
the population covariance matrix is of the order $\sqrt{\log p/n}$. Hence, if $\hat{G}$ (obtained from 
Algorithm \ref{GibbsBSSC}) is an accurate estimate of the true underlying graph $G$ for the true precision matrix 
$\mathbf{\Omega}_0$, we expect that the mode of the refitted posterior density in (\ref{refitted:posterior:density}), given by 
$$
\hat{\mathbf{\Omega}}_{mode, refitted} = \mbox{arg min}_{\mathbf{\Omega} \in \mathbb{M}_{\hat{G}}} \left\{ \frac{n}{2} \text{tr} 
\left( \mathbf{\Omega}^2 S \right) - n \text{tr} (\mathbf{\Omega}) 
\right\}, 
$$

\noindent
is close to $\mathbf{\Omega}_0$. This heuristic analysis is formalized in a high-dimensional setting in 
Theorem \ref{estimation:consistency:refitted:posterior}. 

It follows from Lemma \ref{propriety} that the mode of the refitted posterior density is available in closed from. To compute 
credible intervals, we observe that the full conditional posterior densities of the non-zero elements in 
$\mathbb{M}_{\hat{G}}$ can be derived in a straightforward way. Let $\hat{E}$ denote the edge set for $\hat{G}$. 
In particular, it can be shown that the full conditional (refitted) posterior density of $\omega_{jk}$ for $(j,k) \in \hat{E}$ is 
\begin{equation}
N \left( -\frac{b_{jk}}{a_{jk}}, \frac{1}{na_{jk}} \right)
\end{equation}

\noindent
where 
\begin{equation*}
\begin{split}
a_{jk} &= s_{jj} + s_{kk} , \quad \quad \quad 
b_{jk} = \sum_{k' \neq k, (j,k') \in E} \omega_{jk'}' s_{kk'} + \sum_{j' \neq j, (j',k) \in E} \omega_{j'k} s_{jj'}. \end{split}
\end{equation*}

\noindent
Also the full conditional (refitted) posterior density of $\omega_{jj}$ is 
\begin{equation}
truncN(\frac{1- b_{j}}{s_{jj}}, \frac{1}{ns_{jj}}, 0, \infty),
\end{equation}

\noindent
where 
\begin{equation*}
b_{j} = \sum_{j' \neq j, (j,j') \in E} \omega_{jj'}' s_{jj'}
\end{equation*}

\noindent
and $truncN(\mu, \sigma^2, u, v)$ denotes a normal distribution with mean $\mu$ and variance $\sigma^2$, truncated 
in the interval $(u, v)$. Hence, one can generate approximate samples from the refitted posterior density using a 
Gibbs sampling approach. These samples can then be used to generate a posterior credible region. 

As discussed previously, the refitted posterior density is supported on $\mathbb{M}_{\hat{G}}$, and hence the mode/mean 
is not guaranteed to be positive definite. However, in our numerical analysis, we noticed that as long as the sample size is not 
too small i.e. $n>p/2$, the resulting estimated precision matrix will actually be positive definite.

In case the sample size was really small the resulting estimated precision matrix may not be positive definite. In such 
circumstances, a crude but simple solution, if needed, is to ``project'' the posterior mode/mean (and the associated credible 
region) on the space of positive definite matrices by using the following transformation 
$$
B(\mathbf{\Omega}) = \begin{cases}
\mathbf{\Omega} & \mbox{if } \mathbf{\Omega} \mbox{ is positive definite}, \cr
\mathbf{\Omega} -  \lambda_{\min} (\mathbf{\Omega}) I_p + \epsilon I_p & \mbox{ if } \lambda_{\min} (\mathbf{\Omega}) \leq 0. 
\end{cases}
$$

\noindent
Here $\epsilon > 0$ is a user-defined small positive number. The function $B$ leaves positive definite matrices in 
$\mathcal{M}_{\hat{G}}$ invariant, and appropriately bumps up the diagonal entries of matrices which are not 
positive definite. 

As mentioned previously, the main goal of this paper is selecting the sparsity pattern in $\mathbf{\Omega}$. The refitting and 
projection based method developed in this section for estimating the magnitude of the non-zero entries (post sparsity 
selection) performs well in the simulations in Section \ref{simulations}, and indeed reduces bias. Developing more 
sophisticated, and yet computationally effective methods for projecting into the space of (sparse) positive definite matrices is a 
topic of current research. 



\section{High Dimensional Sparsity Selection Consistency and Convergence Rates for Bayesian Spike-and-Slab CONCORD} 
\label{sec:consistency}

\noindent
In this section, we establish high-dimensional selection and estimation consistency properties of the BSSC approach. We will 
consider a high-dimensional setting, where the number of variables $p = p_n$ increases with the sample size $n$. We will 
assume that the observations ${\bf y}_{1:}^n, {\bf y}_{2:}^n, \cdots, {\bf y}_{n:}^n \in \mathbb{R}^{p_n}$ are i.i.d. with mean 
${\bf 0}$ and precision matrix $\mathbf{\Omega}^0_n$. Let $\boldsymbol{t} = \boldsymbol{t}_n \in \{0,1\}^{{p \choose 2}}$ 
denote the sparsity pattern in the true precision matrix $\mathbf{\Omega}^0_n$, and $d_{\boldsymbol{t}, n}$ denote the 
number of non-zero entries in $\boldsymbol{t}$. For ease of exposition, we will often suppress the dependence of the 
quantities $p_n, \mathbf{\Omega}^0_n, \boldsymbol{t}_n, d_{\boldsymbol{t}, n}$ on $n$, and simply denote them by $p, 
\mathbf{\Omega}^0, \boldsymbol{t}, d_{\boldsymbol{t}}$ respectively. 

Recall from (\ref{theta}) and (\ref{delta}) that ${\boldsymbol \xi}$ and $\boldsymbol{\delta}$ denote the vectorized versions 
of the off-diagonal and diagonal entries of $\mathbf{\Omega}$. Let ${\boldsymbol \xi}^0$ denote the vectorized 
version of the off-diagonal elements of the true precision matrix $\mathbf{\Omega}^0$. Using (\ref{prior on theta}), 
(\ref{prior on delta}), (\ref{BSSC posterior}), and straightforward calculations, the generalized posterior distribution in 
terms of the $({\boldsymbol \xi}, \boldsymbol{\delta})$ can be expressed as 
\begin{eqnarray}
\pi \left\{ {\boldsymbol \xi}, \boldsymbol{\delta} \mid \mathcal{Y} \right\}
& \propto \exp \left\{ n \boldsymbol{1}'\log \left( \boldsymbol{\delta} \right) - \frac{n}{2}\left[ \left( {\begin{array}{*{20}{c}}
{{\boldsymbol \xi}'} &
{\boldsymbol{\delta}'} \\
\end{array} } \right) \left( {\begin{array}{*{20}{c}}
{\mathbf{\Phi}} & {\mathbf{A}} \\
{\mathbf{A}'} & {\mathbf{D}} \\
\end{array} } \right) \left( {\begin{array}{*{20}{c}}
{{\boldsymbol \xi}} \\
{\boldsymbol{\delta}} \nonumber\\
\end{array} } \right) \right] \right\}  \exp \left(-\frac{{\boldsymbol \xi}'\mathbf{\Lambda}{\boldsymbol \xi}}{2} \right) \\
 &\times \sum\limits_{ \boldsymbol{l} \in \mathcal{L}} \left\{ \frac{|\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}} |^{\frac{1}{2}}}{\left(2\pi \right)^{\frac{d_{\boldsymbol{l}}}{2}}} I_{\left( {\boldsymbol \xi} \in \mathcal{M}_{\ell}\right)}\left[ q^{d_{\boldsymbol{l}}}(1-q)^{\binom{p}{2} - d_{\boldsymbol{l}}} \right]\right\} \exp \left( -\gamma \boldsymbol{1}'\boldsymbol{\delta} \right). \label{posterior theta and delta}
\end{eqnarray}

\noindent
where, $\mathbf{\Phi}$ is a $\frac{p(p-1)}{2} \times \frac{p(p-1)}{2}$ symmetric matrix which after indexing the rows and 
columns using $(12, 13, ..., p-1p)$, is given by 
\begin{equation}\label{upsilon}
\mathbf{\Phi}_{\left(ab, cd\right)} = \left\{
	\begin{array}{ll}
		s_{aa} + s_{bb}  & \mbox{if } a=b \ \& \ c=d , \\
				s_{ac}  & \mbox{if } b=d \ \& \ a \neq c,\\
						s_{bd}  & \mbox{if } a=c \ \& \ b\neq d,\\
								0  & \mbox{if } a \neq b \ \& \ c \neq d ,\\
	\end{array}
\right. \quad \text{for} \quad 1 \leq a < b \leq p, \ \text{and} \ 1 \leq c < d \leq p. 
\end{equation}

\noindent
For example, when $p=5$, $\mathbf{\Phi}$ is given as follows. 
\begingroup\makeatletter\def\f@size{8}\check@mathfonts\begin{equation*}
\left( {\begin{array}{*{20}{c}}
{s_{11} + s_{22}} & {s_{23}} & {s_{24}} & {s_{25}} & {s_{13} } & {s_{14} } & {s_{15} } & {0} & {0} & {0} \\ 
{s_{23} } & {s_{11} +s_{33} } & {s_{34} } & {s_{35} } & {s_{12} } & {0} & {0} & {s_{14} } & {s_{15} } & {0} \\ 
{s_{24} } & {s_{34} } & {s_{11}  + s_{44} } & {s_{45} } & {0} & {s_{12} } & {0} & {s_{13} } & {0} & {s_{15} } \\ 
{s_{25} } & {s_{35} } & {s_{45} } & {s_{11} +s_{55} } & {0} & {0} & {s_{12} } & {0} & {s_{13} } & {s_{14} } \\ 
{s_{13} } & {s_{12} } & {0} & {0} & {s_{22} +s_{33} } & {s_{34} } & {s_{35} } & {s_{24} } & {s_{25} } & {0} \\ 
{s_{14} } & {0} & {s_{12} } & {0} & {s_{34} } & {s_{22} +s_{44} } & {s_{45} } & {s_{23} } & {0} & {s_{25} } \\ 
{s_{15} } & {0} & {0} & {s_{12} } & {s_{35} } & {s_{45} } & {s_{22} +s_{55} } & {0} & {s_{23} } & {s_{24} } \\ 
{0} & {s_{14} } & {s_{13} } & {0} & {s_{24} } & {s_{23} } & {0} & {s_{33} +s_{44} } & {s_{45} } & {s_{35} } \\ 
{0} & {s_{15} } & {0} & {s_{13} } & {s_{25} } & {0} & {s_{23} } & {s_{45} } & {s_{33} +s_{55} } & {s_{34} } \\ 
{0} & {0} & {s_{15} } & {s_{14} } & {0} & {s_{25} } & {s_{24} } & {s_{35} } & {s_{34} } & {s_{44} +s_{55} } \\ 
\end{array} } \right),
\end{equation*}
\endgroup

\noindent
In addition, the vector $\boldsymbol{a}$ is a vector of length $\frac{p(p-1)}{2}$ given by 
\begin{equation}\label{a}
\boldsymbol{a}=(s_{12}(\omega_{11}+\omega_{22}), ..., s_{1p} (\omega_{11}+\omega_{pp}),..., s_{p-1p}(\omega_{p-1p-1}+
\omega_{pp}))',
\end{equation}

\noindent
$\mathbf{A}$ is a $\frac{p(p-1)}{2}\times p$ matrix such that $\mathbf{A}\boldsymbol{\delta} = \boldsymbol{a}$ and $\mathbf{D}$ is 
a $p \times p$ diagonal matrix with entries $\left\{ s_{ii} \right\}_{1 \leq i \leq p}$. Recall that $\mathcal{L}$ denotes the space 
of all the $2^{{p \choose 2}}$ sparsity patterns for ${\boldsymbol \xi}$, and $\mathcal{M}_{\boldsymbol{l}}$ denotes the 
space in which the parameter ${\boldsymbol \xi}$ varies when restricted to the sparsity pattern $\boldsymbol{l}$. 

%while that of $\boldsymbol{\delta}$ given ${\boldsymbol \xi}$ has the following form,
%\begin{equation}\label{posterior delta given theta}
%\begin{split}
%\pi \left\{ \boldsymbol{\delta} | {\boldsymbol \xi}, \mathcal{Y}\right\} \propto \prod\limits_{i=1}^p \left( \omega_{ii}\right)^n \exp \left\{ -\frac{n}{2} s_{ii}\left( \omega_{ii}\right)^2 - \left(\gamma + n\sum_{j \ne i}{\omega_{ij}s_{ij}}\right) \omega_{ii}\right\}.
%\end{split}
%\end{equation}

Note that our main objective is to accurately estimate the off-diagonal entries. Hence, as commonly done for generalized 
likelihood based high-dimensional consistency proofs - see \cite{khare2015convex,peng2009partial} - we assume the 
existence of accurate estimates for the diagonal elements, i.e., there exist estimates $ \hat{\omega}_{ii}$, such that for any 
$\eta>0$, there exists a constant $C>0$, such that 
\begin{equation} \label{accurate-estimation}
\max_{ 1 \leq k \leq K} \| \hat{\omega}_{ii} - \omega_{ii}\| \leq C \left( \sqrt{\frac{\log p}{n}}\right),
\end{equation}

\noindent
with probability at least $1-O(n^{-\eta})$. One way to get such estimates of the diagonal entries is discussed in Lemma 4 of 
\cite{khare2015convex}. Denote the resulting estimates of the vectors $\boldsymbol{\delta}$ and $\boldsymbol{a}$ by 
$\hat{\boldsymbol{\delta}}$ and $\hat{\boldsymbol{a}}$, respectively. We now consider the accuracy of the estimates of the 
off-diagonal entries obtained after running the BSSC procedure with the diagonal entries fixed at $\hat{\boldsymbol{\delta}}$. 
Please also see Remark \ref{implication of assumption 1} for the implication of this assumption on the posterior contraction 
rate in Theorem 2. For this section, we will assume that the entries of $\mathbf{\Lambda}$ are fixed. 

Now, in view of (\ref{posterior theta and delta}), the conditional posterior distribution of the off-diagonal entries vector 
${\boldsymbol \xi}$ given $\hat{\boldsymbol{\delta}}$ is given as follows. 
\begin{equation}\label{posterior theta given delta}
\begin{split}
&\pi \left\{ {\boldsymbol \xi} |\hat{\boldsymbol{\delta}}, \mathcal{Y}\right\} \propto \exp \left\{ - \frac{1}{2}\left[ 
{\boldsymbol \xi}'\left( n\mathbf{\Phi} + \mathbf{\Lambda}\right) {\boldsymbol \xi} + 2n{\boldsymbol \xi}' 
\hat{\boldsymbol{a}} \right] \right\} \\
&\times \sum\limits_{ \boldsymbol{l} \in \mathcal{L}} \left\{ \frac{|\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}}|^{\frac{1}{2}}}{\left(2\pi \right)^{\frac{d_{\boldsymbol{l}}}{2}}} I_{\left( {\boldsymbol \xi} \in \mathcal{M}_{\boldsymbol{l}}\right)}  \left[ q^{d_{\boldsymbol{{\boldsymbol{l}}}}}(1-q)^{\binom{p}{2} - d_{\boldsymbol{l}}} \right]\right\},
\end{split}
\end{equation}

\noindent
The above posterior distribution is a mixture distribution, and induces a posterior distribution on the space of sparsity patterns. 
In particular, by straightforward calculations (see proof of Lemma S4 in the Supplemental document) we get that 
\begin{equation} \label{eqsparsity}
\pi \left\{ \boldsymbol{l} | \hat{\boldsymbol{\delta}}, \mathcal{Y} \right\} \propto q^{d_{\boldsymbol{l}}}(1-q)^{\binom{p}{2} - d_{\boldsymbol{l}}} \frac{|\mathbf{\Lambda}_{\boldsymbol{l}\boldsymbol{l}}|^{\frac{1}{2}}}{| \left( n\mathbf{\Phi} + \mathbf{\Lambda}\right)_{{\boldsymbol{l}}{\boldsymbol{l}}}|^{\frac{1}{2}}} \exp\left\{ \frac{n^2}{2}\hat{\boldsymbol{a}}_{\boldsymbol{l}}' \left( n\mathbf{\Phi} + \mathbf{\Lambda}\right)_{{\boldsymbol{l}}{\boldsymbol{l}}}^{-1}\hat{\boldsymbol{a}}_{\boldsymbol{l}}\right\}. 
\end{equation}

\noindent
for every ${\boldsymbol \ell} \in \mathcal{L}$. Our main goal in this section is to study the high-dimensional asymptotic 
properties of this posterior distribution on the space of sparsity patterns. We make the following standard and mild regularity 
assumptions before presenting our consistency results. 
\begin{Assumption}\label{Assumption2: d_t} 
$d_{\boldsymbol{t}} \sqrt{\frac{\log p}{n}} \to 0, \quad \quad \text{as} \quad n \to \infty$. 
\end{Assumption}

\noindent
This assumption essentially states that the number of variables $p$ has to grow slower than 
$e^{(\frac{n}{d_{\boldsymbol{t}}^2})}$. Similar assumptions have been made in other high dimensional covariance estimation 
methods e.g. \cite{banerjee2014posterior}, \cite{banerjee2015bayesian}, \cite{bickel2008regularized}, and 
\cite{xiang2015high}.

\begin{Assumption}\label{Assumption4: Sub-Gaussianity} There exists $c>0$, independent of $n$ such that 
\begin{equation*}
\mathbb{E}_0 \left[ \exp \left( {\boldsymbol{\alpha}'\mathbf{y_{i:}}} \right) \right] \leq \exp \left( c \boldsymbol{\alpha}' 
\boldsymbol{\alpha} \right).
\end{equation*}
\end{Assumption}

\noindent
Here $\mathbb{E}_0$ denotes the expected value with respect to the true data generating model. The above assumption 
allows for deviations from Gaussianity. Hence, Theorem \ref{theorem (strong consistency)} below will show that the BSSC 
procedure is robust (in terms of consistency) under misspecification of the data generating distribution, as long as its tails are 
sub-Gaussian. 

\begin{Assumption}\label{Assumption3: Bounded eigenvalues}
(Bounded eigenvalues). There exists $\tilde{\varepsilon_{0}} > 0$, independent of $n$, such that 
\begin{equation*}
\tilde{\varepsilon_{0}} \leq \text{eig}_{\min}\left( {\mathbf{\Omega}}^0 \right) \leq \text{eig}_{\max}\left( {\mathbf{\Omega}}^0 
\right) \leq \frac{1}{\tilde{\varepsilon_{0}}}.
\end{equation*}
\end{Assumption}

\noindent
This is a standard assumption in high dimensional analysis to obtain consistency results, see for example  
\cite{buhlmann2011statistics}. 

Henceforth, we let $\varepsilon_{0} = c^2\tilde{\varepsilon_{0}}$, $a_1 = \frac{\varepsilon_0^3}{768 }$, 
$a_2 = \frac{8c^2}{\varepsilon_0}$. 

\begin{Assumption}\label{Assumption5: Signal Strength}
(Signal Strength). Let $s_n$ be the smallest non-zero entry (in magnitude) in the vector ${\boldsymbol \xi}_0$. We assume 
$\frac{\frac{1}{2}\log n + a_2d_{\boldsymbol{t}}\log p}{a_1 n s_n^2} \to 0$.
\end{Assumption}

\noindent
This is again a standard assumption. Similar assumptions on the appropriate signal size can be found in 
\cite{khare2015convex,peng2009partial}. 

\begin{Assumption}\label{Assumption6: Decay rate} (Decay rate of the edge probabilities).
Let $q = p^{-a_2 d_{\boldsymbol{t}}}$. 
\end{Assumption}

This can be interpreted as a priori penalizing sparsity patterns with too many non-zero entries. We now establish the main 
posterior consistency result. In particular, we show that the posterior mass assigned to the true sparsity pattern converges to 
one in probability (under the true model), if we restrict to {\it realistic sparsity patterns}, i.e., sparsity patterns where the 
number of non-zero entries is bounded by $\tau_n = \frac{\varepsilon_0}{4c}\sqrt{\frac{n}{\log p}}$. 

\begin{Theorem}\label{theorem (strong consistency)}
(Strong Selection Consistency) Under Assumptions \ref{Assumption2: d_t} - \ref{Assumption6: Decay rate}, and restricting to 
realistic sparsity patterns, the posterior distribution on the sparsity patterns in (\ref{eqsparsity}) puts all of its mass on the true 
sparsity pattern ${\bf t}$ as $n \rightarrow infty$, i.e., 
\begin{enumerate}
\item 
\begin{equation}\label{main result}
\pi \left\{ \boldsymbol{t} | \hat{\boldsymbol{\delta}},\mathcal{Y}\right\} 
\xrightarrow{\text{$\mathbb{P}_0$}} 1, \quad \quad \text{as} \quad n \to \infty.
\end{equation}

\item The sparsity pattern estimate $\hat{\boldsymbol{l}}_{\upsilon, BSSC}$, obtained by using the output of the BSSC 
algorithm and applying the thresholding approach discussed at the end of Section \ref{posterior:computation:gibbs:sampler}, 
satisfies 
$$
\mathbb{P}_0 \left( \hat{\boldsymbol{l}}_{\upsilon, BSSC} = \boldsymbol{t} \right) \rightarrow 1 \quad \quad \text{as} \quad n 
\to \infty. 
$$
\end{enumerate}
\end{Theorem}

\noindent
While our main goal is sparsity selection consistency, we also derive two results that establish estimation consistency/
convergence rates for (i) the estimates of the magnitudes of the non-zero entries obtained directly from the BSSC algorithm 
(Algorithm \ref{GibbsBSSC}) (Theorem \ref{theorem (Estimation Consistency and Convergence Rate)}), and (ii) the estimates 
of the magnitudes of the non-zero entries obtained from the refitted posterior density defined in (\ref{refitted:posterior:density}). 
\begin{Theorem}\label{theorem (Estimation Consistency and Convergence Rate)}
(Estimation Consistency Rate) Let $R_n$ be the maximum value (in magnitude) in the vector ${\boldsymbol \xi}^0$ and 
assume that $R_n$ can not grow at a rate faster than $\sqrt{n \log p}$. Then, based on the joint posterior distribution given 
in (\ref{posterior theta and delta}), and under Assumptions \ref{Assumption2: d_t} - \ref{Assumption6: Decay rate}, there 
exists a large enough constant $G$ (not depending on $n$), such that the following holds. 
\begin{equation}
\mathbb{E}_{0} \left[\pi \left(\| {\boldsymbol \xi} - {\boldsymbol \xi}^0\|_2 > G \sqrt{\frac{d_{\boldsymbol{t}} \log p}{n}} \mid 
\hat{\boldsymbol{\delta}}, \mathcal{Y}\right) \right] \quad \to 0 \quad \text{as} \quad n \to \infty.
\end{equation}
\end{Theorem}

\begin{Theorem} \label{estimation:consistency:refitted:posterior}
(Estimation Consistency for refitted posterior mode) Under the same assumptions as in 
Theorem \ref{theorem (Estimation Consistency and Convergence Rate)}, the mode $\hat{\mathbf{\Omega}}_{refitted}$ of 
the refitted posterior density in (\ref{refitted:posterior:density}) satisfies 
$$
\mathbb{P}_{0} \left( \left\| \hat{\mathbf{\Omega}}_{refitted} - \mathbf{\Omega}^0 \right\| > G' \sqrt{\frac{d_{\boldsymbol{t}} 
\log p}{n}} \right) \rightarrow 0 \quad \quad \mbox{as} n \quad \to \infty, 
$$

\noindent
for a large enough constant $G'$ (not depending on $n$). 
\end{Theorem}

\noindent
The proofs of the three results above are provided in the Supplemental Section S3. 

\begin{Remark}\label{implication of assumption 1}
Posterior estimation  consistency/contraction rates for some pseudo-likelihood based Bayesian approaches have been 
studied in recent work by \cite{atchade2017contraction}. In particular, a {\it single binary} graphical model (as opposed 
to multiple Gaussian graphical models in our setting) is one of the settings considered in \cite{atchade2017contraction}. 
For this setting, a posterior contraction rate of $\sqrt{\frac{(p + d_t) \log p}{n}}$ for $\Omega$ (including both the 
diagonal and off-diagonal entries) in Frobenius norm is obtained without making an assumption similar to our assumption 
of accurate diagonal estimates (as compared to the rate of $\sqrt{\frac{d_t \log p}{n}}$ for only the off-diagonal entries in 
Theorem 2, which uses this assumption). Note that results in \cite{atchade2017contraction} do not address model selection 
consistency.  
\end{Remark} 



\section{Simulation Studies}\label{simulations}

\noindent
In this section, we evaluate accuracy, computational speed and scalability of our model. As mentioned earlier, the main 
challenge with existing Bayesian methodologies is their limited scalability. To the best of our knowledge, 
Stochastic Search Structure Learning (SSSL) introduced in \cite{Wang:2015}, is the fastest Bayesian covariance 
selection method (see Section 5 of \cite{Wang:2015}). Hence, we use SSSL as a benchmark for the performance of our 
BSSC method. 

\subsection{Computational scalability: Timing and memory requirement comparison} \label{computation}

\noindent
For the purposes of assessing computational scalability, we use $p \in \{150, 300, 500, 1000, 3000\}$. For each $p$,  the {\it true} 
precision matrix $\mathbf{\Omega}^0$ is chosen to have a complete random sparsity patterns with $4 \%$ edge density. 
The non-zero off-diagonal entries generated from $[-0.6, -0.4] \cup [0.4, 0.6]$, and the diagonal entries are adjusted 
as needed to make the resulting matrix positive definite. We then generate $25$ replicate datasets of size $n = p/2$ from a 
multivariate Gaussian distribution with mean ${\bf 0}$ and precision matrix $\mathbf{\Omega}^0$. For each dataset, we run 
the BSSC (with default hyperparameter values as discussed in Remark \ref{hyperparameter:selection}), SSSL (with 
default hyperparameter values as specified in \cite{Wang:2015} and Glasso (with the final value of its shrinkage parameter manually selected using exhaustive cross-validations) methods. 


For BSSC, we used 2000 iterations of 
Algorithm \ref{GibbsBSSC} as burn-in, and 2000 more iterations to generate our estimates (standard diagnostics indicated 
that these number of iterations were enough for convergence). For SSSL and with $p \in \{150, 300\}$, we used the default setting in \cite{Wang:2015} 
of 1000 iterations for burn-in, and 10000 iterations for computing posterior estimates, however for higher dimensions e.g. $p \in \{500, 1000, 3000\}$, the default setting required more than 50 GigaBytes of memory thus due to memory limitations, we iterated the model 500 iterations during each states of burn-in and computing posterior estimates. Finally, the results for Glasso were achieved using default number of iterations. To ensure a fair comparison, we compare the two algorithms below in terms of {\it time taken per iteration}. The simulations were performed using 
dedicated cores of the HPC (High Performance Computing) cluster at the University of Florida. 

We provide the {\it time taken per iteration} for BSSC, SSSL, and Glasso averaged over 25 replications in Table \ref{wall_time} below. The results demonstrate that SSSL struggles computationally even when $p = 500$, while BSSC easily handles sittings with thousands of nodes, most notably for $p = 3000$, BSSC iterates in less than 44 seconds which is over 5760 times faster than SSSL. Furthermore, BSSC iterates mush faster than Glasso making them computationally comparable, especially for estimating precision matrices with lower hundred $p$s. However as $p$ grows, Glasso still has the time advantage, since it requires only less than 10 iterations to converge.


\begin{table}[h]
\centering 
\caption{Average wall-clock seconds per iteration for BSSC, Glasso, and SSSL for estimating a $p \times p$ precision matrix 
with $p \in (150, 300, 500, 1000 \ \text{and} \ 3000)$.}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 &{$p=150$}&{$p=300$}&{$p=500$}&{$p=1000$} &{$p=3000$}\\
\midrule
{BSC} & {0.006} & {0.035} & {0.112} & {0.675} &{43.122}  \\
\midrule
{Glasso} & {0.108} & {0.293} & {0.523 } & {5.857} &{168.333} \\
\midrule
{SSSL} & {0.104} & {1.31} & {10.1} & {37.38} & {237600} \\
\bottomrule
\end{tabular}}
\label{wall_time}
\end{table}


In addition, the memory usage of BSSC is significantly less than SSSL. The average memory used by BSSC and SSSL for 
different values of $p$ is summarized in Table \ref{memory usage}. Note that SSSL requires more than 50 GB for $p \geq 500$ while BSSC achieves the goal with 0.24 GB of memory. 
\begin{table}[h]
\centering 
\caption{Average GigaByte memory usage for BSSC and SSSL for estimating a $p \times p$ precision matrix with $p \in 
(150, 300, 500, 1000 \ \text{and} \ 3000)$.}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 &{$p=150$}&{$p=300$}&{$p=500$}&{$p=1000$}&{$p=3000$}\\
\midrule
{BSC} & {0.001} & {0.22} & {0.24} & {0.32} & {1.39}  \\
\midrule
{SSSL} & {5.3} & {20.4} & {$>$50 } & {$>$50}& {$>$50} \\
\bottomrule
\end{tabular}}
\label{memory usage}
\end{table}

\noindent
The reason for the substantially superior performance of BSSC as compared to the SSSL becomes apparent after a study 
of the computational complexity per iteration of both algorithms. The SSSL algorithm requires $2(p-1)$ matrix inversions of 
$(p-1) \times (p-1)$ matrices (see Section 4.1 of \cite{Wang:2015}). The worst case computational complexity for one 
iteration of the SSSL algorithm therefore is $O(p^4)$. On the other hand, in the worst case, one iteration on the BSSC 
algorithm has computational complexity $O(p^3)$ (update each of the ${p \choose 2}$ entries with $O(p)$ computations, 
see Algorithm \ref{GibbsBSSC}), and {\bf no matrix inversions} are needed. When the precision matrices generated/used in 
the iterates of these algorithms are sparse, the computational complexity for both BSSC and SSSL will improve. Even in this 
sparse setting, as demonstrated by the simulations above, BSSC is orders of magnitude faster than SSSL. In fact, the effect 
of sparsity in $\mathbf{\Omega}$ on BSSC is clear: the inner products of the form $\mathbf{\Omega}_{-jk}'\mathbf{S}_{-jj}$ 
used in the updates can be computed faster if $\mathbf{\Omega}_{-jk}$ is 
Additionally, the matrix inversions needed for 
SSSL also create substantial memory requirements even in moderate/high dimensional settings, as demonstrate by the 
simulation above for $p = 500$ and $p = 1000$. 

\subsection{Statistical accuracy comparison} \label{accuracy}

\noindent
We now assess the sparsity selection accuracy of our model and compare with SSSL using three well known accuracy 
measures, specificity (SP), sensitivity (SE) and Matthews Correlation Coefficients (MCC) defined as:
\begin{equation}\label{accuracy measures}
\begin{split}
\text{SP} &= \frac{\text{TN}}{\text{TN} + \text{FP}}, \quad \quad \quad \text{SE} = \frac{\text{TP}}{\text{TP} + \text{FN}}\\
\text{MCC} &= \frac{\text{TP} \times \text{TN} - \text{FP} \times \text{FN}}{\sqrt{(\text{TP} + \text{FP})(\text{TP} + \text{FN})(\text{TN} + \text{FP})(\text{TN} + \text{FN})}}
\end{split}
\end{equation}

\noindent
where, TP, TN, FP and FN represent the number of true positives, true negatives, false positives and false negatives, 
respectively. Larger values of any of the above metrics indicates a better sparsity selection produced by the underlying 
method. In our comparison, we include precision matrices with dimensions $p \in (150, 300, 500, \text{and} \ 1000)$, and 
sample sizes $n \in (p/2, 3p/4, p, \text{and} \ 2p)$. We also consider two matrix density (the proportion of the non-zero edges 
in the upper (lower) off-diagonal elements) levels of 0.04 and 0.1 for the true precision matrix $\mathbf{\Omega}^0$. We 
generate $\mathbf{\Omega}^0$ using the same mechanism as in Section \ref{computation}. For each combination of $p$, 
$n$, and edge density level, we generate $50$ replicate datasets of size $n$ from a multivariate normal distribution with 
mean ${\bf 0}$ and precision matrix $\mathbf{\Omega}^0$.For each dataset, we obtain the sparsity pattern estimate 
for $\mathbf{\Omega}$ using both BSSC and SSSL, and obtain the SP, SE, MCC values by comparing to the true 
sparsity pattern in $\mathbf{\Omega}^0$. Again, for BSSC, we used 2000 iterations of Algorithm \ref{GibbsBSSC} as 
burn-in, and 2000 more iterations to generate our estimates (standard diagnostics indicated that these number of iterations 
were enough for convergence). For SSSL with small number of nodes e.g. $p \in \{150, 300\}$, we used the default setting in \cite{Wang:2015} 
of 1000 iterations for burn-in, and 10000 iterations for computing posterior estimates, however unfortunately, as $p$ grows moderately, the computational 
cost of SSSL grows very quickly, as demonstrated by Table \ref{wall_time} and Table \ref{memory usage}. For instance, even 
for a moderate size problem with $p=500$, the SSSL requires more than $50$ Gigabyte of memory to run the default number of iterations which is $11000$. Due to this limitation and the associated computational burden, we were not able to run the default settings of SSSL for precision matrices with $p=500$ and 
$p=1000$. Consequently, to achieve results for $p=500$ and 
$p=1000$ with SSSL, we iterated it 500 times during each states of burn-in and computing posterior estimates.


The SP, SE, MCC values, averaged over all the $50$ replicate 
datasets, are provided in Table \ref{comparing SSSL and BSSC}. Overall, a comparison of the MCC values in Table \ref{comparing SSSL and BSSC} demonstrates better sparsity selection 
performance by BSSC compared to SSSL when the edge density of the true precision matrices is $0.1$, while the results are 
comparable when the edge density of the true precision matrices in $0.04$. {\it The results in this section, and in 
Section \ref{computation} demonstrate that BSSC can lead to substantial improvement in computational performance 
compared to SSSL, while improving/maintaining sparsity selection accuracy}. 
\begin{table}[H]
\centering 
\caption{Average sparsity selection accuracy for BSSC and SSSL for estimating a $p \times p$ precision matrix with 
$p \in (150, 300, 500, \text{and} \ 1000)$.}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
 &&&&{BSSC}&&&&{SSSL}&\\
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
 & & {$p=150$} & {$p=300$} & {$p=500$} & {$p=1000$} & {$p=150$} & {$p=300$} & {$p=500$} & {$p=1000$} \\
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10}   
$n$ &&&&{$Density = 0.04$}&&&&{$Density = 0.04$}&\\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$p/2$} } 
& {SP\%}& {99} & {100} & {100} & {100} & {100} & {100} & {100} & {100}   \\
& {SE\%}& {26} & {28} & {29} & {30} & {20} & {22} & {17} & {17}   \\
& {MC\%}& {41} & {44} & {45} & {46} & {39} & {42} & {37} & {36}   \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$3p/4$} } 
& {SP\%}& {99} & {100} & {100} & {100} & {100} & {100} & {100} & {100}    \\
& {SE\%}& {41} & {43} & {45} & {47} & {34} & {35} & {29} & {28}   \\
& {MC\%}& {55} & {58} & {60} & {62} & {54} & {56} & {50} & {49} \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$p$} } 
& {SP\%}& {100} & {100} & {100} & {100} & {100} & {100} & {100} & {100}   \\
& {SE\%}& {53} & {57} & {60} & {61} & {45} & {48} & {41} & {38}   \\
& {MC\%}& {67} & {70} & {71} & {73} & {64} & {67} & {61} & {58}  \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$2p$} } 
& {SP\%}& {100} & {100} & {100} & {100} & {100} & {100} & {100} & {100}   \\
& {SE\%}& {86} & {89} & {91} & {92} & {78} & {85} & {79} & {74}    \\
& {MC\%}& {89} & {91} & {92} & {93} & {87} & {91} & {88} & {85}   \\
\midrule
$n$ &&&&{$Density = 0.1$}&&&&{$Density = 0.1$}&\\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$p/2$} } 
& {SP\%}& {99} & {99} & {99} & {99} & {100} & {100} & {100} & {100}    \\
& {SE\%}& {12} & {11} & {10} & {11} & {9} & {4} & {6} & {5}    \\
& {MC\%}& {24} & {24} & {23} & {24} & {23} & {16} & {19} & {17}   \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$3p/4$} } 
& {SP\%}& {99} & {99} & {99} & {99} & {100} & {100} & {100} & {100}    \\
& {SE\%}& {18} & {17} & {17} & {18} & {15} & {9} & {11} & {9}   \\
& {MC\%}& {33} & {33} & {32} & {33} & {33} & {25} & {28} & {24}    \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$p$} } 
& {SP\%}& {99} & {99} & {99} & {99} & {100} & {100} & {100} & {100}   \\
& {SE\%}& {25} & {24} & {23} & {25} & {21} & {13} & {16} & {13}   \\
& {MC\%}& {40} & {41} & {40} & {41} & {40} & {31} & {34} & {29}   \\
\cmidrule(lr){1-2}  
\cmidrule(lr){3-6} 
\cmidrule(lr){7-10} 
{\multirow{3}{*}{$2p$} } 
& {SP\%}& {99} & {99} & {99} & {99} & {100} & {100} & {100} & {100}    \\
& {SE\%}& {49} & {49} & {48} & {51} & {44} & {30} & {35} & {27}   \\
& {MC\%}& {63} & {64} & {63} & {65} & {62} & {51} & {55} & {47}   \\
\bottomrule
\end{tabular}}
\label{comparing SSSL and BSSC}
\end{table}

\noindent
While our main goal is sparsity selection, we now examine the effectiveness of the refitting technique developed in 
Section \ref{refitting:technique} for reducing the estimation bias in the magnitude of the non-zero entries. We do so by 
studying the improvements in relative error with respect to the Frobenius norm, namely $\frac{\|\hat{\mathbf{\Omega}} - 
\mathbf{\Omega}^0\|_{F}}{\mathbf{\|\Omega}^0\|_{F}}$, where two choices are used for $\hat{\mathbf{\Omega}}$. Let 
$\hat{E}$ denote the collection of indices chosen as non-zero using the thresholding procedure described at the end of 
Section \ref{posterior:computation:gibbs:sampler}, and $\left\{ \hat{\mathbf{\Omega}}^(t) \right\}_{t=1}^T$ denote 
the sequence of iterates obtained by running the Gibbs sampler in Algorithm \ref{GibbsBSSC}. Our first estimate of 
$\mathbf{\Omega}$ is given by 
\begin{equation} \label{estimate}
\hat{\mathbf{\Omega}}_{BSSC} = \begin{cases}
\frac{\sum_{t=1}^T \hat{\omega}_{jk}^{(t)}}{\sum_{t=1}^T 1_{\{\hat{\omega}_{jk}^{(t)} \neq 0\}}} & \mbox{if } (j,k) \in \hat{E}, 
\mbox{ or } j=k, \cr
0 & \mbox{if } (j,k) \notin \hat{E}. 
\end{cases}
\end{equation}

\noindent
The second estimate, denoted by $\hat{\mathbf{\Omega}}_{refitted}$ is the posterior mean of the refitted posterior density 
in (\ref{refitted:posterior:density}), which can again be computed by the modified Gibbs sampling procedure on 
$\mathbb{M}_{\hat{G}}$ discussed at the end of Section \ref{refitting:technique}. Note that both 
$\hat{\mathbf{\Omega}}_{BSSC}$ and $\hat{\mathbf{\Omega}}_{refitted}$ set the indices not in $\hat{E}$ to be zero, 
and differ only in the magnitudes of indices classified as non-zero, i.e., indices in $\hat{E}$. We consider $p \in (50, 100, 
150, 200, \text{and} \ 300)$, and $n= p$. The true precision matrix $\mathbf{\Omega}^0$ is generated by using the same 
mechanism in Section \ref{computation}, and for each $p$, the relative Frobenius norm of the two estimates described 
above are averaged over $50$ replicate datasets. The results are provided in Table \ref{debiasing sim}, and clearly 
demonstrate the improvement in estimation of the magnitudes by using the refitting technique in 
Section \ref{refitting:technique}, particularly for larger values of $p$. 
\begin{table}[h]
\centering 
\caption{Summary of average relative error for estimation of the magnitudes of the precision matrix entries for estimates 
directly obtained from Algorithm \ref{GibbsBSSC} vs. estimates obtained by using the refitting technique in 
Section \ref{refitting:technique}}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 &{$p=n=50$}&{$p=n=100$}&{$p=n=150$}&{$p=n=200$}&{$p=n=300$}\\
\midrule
{BSSC} & {0.38} & {0.45} & {0.45 } & {0.45 } &  {0.49} \\
\midrule
{BSSC with refitting} & {0.36} & {0.35} & {0.32 } & {0.32 } &  {0.29} \\
\bottomrule
\end{tabular}}
\label{debiasing sim}
\end{table}
 
 
\subsection{Metabolomics data}
 

Integrative Human Microbiome Project.

The data were downloaded from the Metabolomics Workbench \texttt{www.metabolomicsworkbench.org} (Study ID ST000923)

correspond to measurements of 428 primary and secondary metabolites and lipids (289 lipids, 139 proteins)

stool samples of  208 inflammatory bowel disease (IBD) female patients

total edges in the network: 2136



\begin{figure}[h]
\centering
\caption{289 lipids; total edges: 1304; edges with degree bigger than 11 }
  \centering
  \includegraphics[height=3in,width=4in,angle=0]{Net_set_2_2}
  \label{sub net 2}
\end{figure}


\begin{figure}[h]
\centering
\caption{139 proteins; total edges: 412; edges with degree bigger than 8 shown }
  \centering
  \includegraphics[height=3in,width=4in,angle=0]{Net_set_1}
  \label{sub net 1}
\end{figure}



